Neural network execution using nicked DNA and microfluidics

DNA has been discussed as a potential medium for data storage. Potentially it could be denser, could consume less energy, and could be more durable than conventional storage media such as hard drives, solid-state storage, and optical media. However, computing on data stored in DNA is a largely unexplored challenge. This paper proposes an integrated circuit (IC) based on microfluidics that can perform complex operations such as artificial neural network (ANN) computation on data stored in DNA. It computes entirely in the molecular domain without converting data to electrical form, making it a form of in-memory computing on DNA. The computation is achieved by topologically modifying DNA strands through the use of enzymes called nickases. A novel scheme is proposed for representing data stochastically through the concentration of the DNA molecules that are nicked at specific sites. The paper provides details of the biochemical design, as well as the design, layout, and operation of the microfluidics device. Benchmarks are reported on the performance of neural network computation.

==> concentration.tex <==
\subsection{Computation}

This paper demonstrates novel schemes for implementing operations such as multiplication, dot product, and neural functions on data stored in DNA. Computation is effected via the mechanism of of {\em toehold-mediated DNA strand displacement}~\cite{Yurke_2000},~\cite{Soloveichik5393}.

Recent research has shown how data can be encoded via {\em nicks} on DNA using gene-editing enzymes like CRISPR-Cas9 and PfAgo~\cite{Tabatabaei_Wang_Athreya_Enghiad_Hernandez_Leburton_Soloveichik_Zhao_Milenkovic_2019}. 
{\em Probabilistic switching} of concentration values has been demonstrated by the DNA computing community~\cite{Cherry_Qian_2018}. In previous work, we demonstrated how a concept from computer engineering called {\em stochastic logic} can be adapted to DNA computing~\cite{Salehi_Liu_Riedel_Parhi_2018}. In this paper,
we bring these disparate threads together: we demonstrate how to perform stochastic computation on
{\em fractionally-encoded} data stored on nicked DNA.

\subsubsection{Encoding Values}
\label{sec:rep_val}

The conventional approach to storing data in DNA is to use a single species of strand to 
represent a value. It is either encoded as a binary value, where the presence of
the specific strand represents a 1 and its absence a 0~\cite{Seelig1585}; 
or as a non-integer value, encoded according to its concentration, called a {\em direct representation}~\cite{Wilhelm_Bruck_Qian_2018}.
In recent research, we have shown how a {\em fractional representation} can be used~\cite{Salehi_Liu_Riedel_Parhi_2018}. The idea is to use the concentration of two species of strand $X_0, X_1$ to represent a value $x$ with
$$x=\frac{X_1}{X_0+X_1}$$
where $x\in[0,1]$.
This encoding is related to the concept of {\em stochastic
logic} in which computation is performed on randomized bit streams, with values represented by the fraction of 1's versus 0's in the stream~\cite{Gaines1969},~\cite{Qian08-DAC},~\cite{Qian10-TOC}.

In this work, we store values according to nicking sites on double DNA strands. For a given site, we will have some strands nicked there, others not. Let the overall concentration of the double strand equal $C_0$, and the concentration of strands nicked at the site equal $C_1$. The ratio of the concentration of strands nicked versus the overall concentration is
$$x=\frac{C_1}{C_0}$$
So this ratio is the relative concentration of the nicked strand at this site. We use it to represent a  variable $x \in [0,1]$.

Setting this ratio can be achieved by two possible methods. One is that we nick a site using a gene-editing guide that is not fully complementary to the nicking site. The degree of complementarity would control the rate of nicking and so set the relative concentration of strands that are nicked. A simpler method is to split the initial solution containing the strand into two samples; nick all the strands in one sample; and then mix together the two samples with the desired ratio $x$. 

\section{Multiplication}
\label{sec:multiply}

The core component of our design is the multiplication operation. It requires that the presence of nicks at a given sites be statistically independent to the presence of nicks at other sites on the same strand.

\subsection{Multiplying two values}

Multiplying two fractionally encoded values requires two neighboring nicking sites. Suppose we 
have two such sites $A$ and $B$ on a double strand. For each site, there are
two possibilities: nicked or not nicked. Let $a$ and $b$ be the relative concentrations of strands nicked at sites $A$ and $B$, 
respectively. We assume the nicking is done independently. Figure~\ref{fig:mult2} shows four different possible scenarios on a given 
strand. The truth table on the left shows whether a specific location is nicked or not,
and the concentration on the right shows the relative concentration for each scenario.
Here we use the single strand between $A$ and $B$ in the last scenario, shown in red, to represent the result of the multiplication. The concentration of this strand specifies the result since it only appears
 when both sites $A$ and $B$ are nicked. According to our assumption, the presence of nicks at $A$ and $B$ are statistically independent. So the probability that both sites are nicked is $a\times b$. In Section~\ref{sec:readout}, we discuss how to release the single strand between the two sites. Its relative concentration translates to the value of the multiplication operation, $a \times b$.

\begin{figure}[t]
\centering
	\includegraphics[width=\linewidth]{MULT1.pdf}
    \caption{Multiplying two values, $a$ and $b$. The result is the relative concentration of the red strand.}
\label{fig:mult2}
\end{figure} 

\begin{figure}[t]
\centering
	\includegraphics[width=\linewidth]{probe.pdf}
    \caption{Using a {\em probe} strand to read out the result. When a complementary single strand of DNA, called a {\em probe}, shown as the top black strand, is added, it displaces and releases the single strands  from regions in between nicks.}
\label{fig:probeout}
\end{figure} 

\section{Reading Out}
\label{sec:readout}

To process the result of multiplication, we need to detach single strands from the base double strand. The diagram shown in Figure~\ref{fig:probeout} illustrates this process. When a complementary single strand called a {\em probe} is supplied, it will displace and release single strands located between nicks, provided that the distance between nicks is small~\cite{Hayward2108}. In Section~\ref{sec:scaling}, we discuss how these single strands can then participate in further strand-displacement operations.


